Dual Contrastive Learning for General Face Forgery Detection

With various facial manipulation techniques arising, face forgery detection has drawn growing attention due to security concerns. Previous works always formulate face forgery detection as a classification problem based on cross-entropy loss, which emphasizes category-level differences rather than the essential discrepancies between real and fake faces, limiting model generalization in unseen domains. To address this issue, we propose a novel face forgery detection framework, named Dual Contrastive Learning (DCL), which specially constructs positive and negative paired data and performs designed contrastive learning at different granularities to learn generalized feature representation. Concretely, combined with the hard sample selection strategy, Inter-Instance Contrastive Learning (Inter-ICL) is first proposed to promote task-related discriminative features learning by especially constructing instance pairs. Moreover, to further explore the essential discrepancies, Intra-Instance Contrastive Learning (Intra-ICL) is introduced to focus on the local content inconsistencies prevalent in the forged faces by constructing local-region pairs inside instances. Extensive experiments and visualizations on several datasets demonstrate the generalization of our method against the state-of-the-art competitors.

==> old_version/AAAI-method.tex <==
\begin{figure*}[h]
    \begin{center}
    \includegraphics[width=0.9\textwidth]{Figure/mainv5.pdf}
    \end{center}
       \caption{Overview of our proposed method. 
       }
    \label{fig:main}
\end{figure*}

In this section, we firstly introduce the proposed supervised contrastive learning framework for general face forgery detection in Sec.~\ref{section:1}
Then three key components: %\textit{i.e.}%
Image View Transform (IVT), Adaptive Hard Sample Selection strategy (AHSS) and Similarity Contrastive Module (SCM) in Sec.~\ref{section:2} are presented in detail. At last, all the supervised loss functions are summarized in Sec.~\ref{section:3}

\subsection{Overview Framework}
\label{section:1}
The architecture of our proposed method is illustrated in Fig~\ref{fig:main}. In order to guide the network to learn more general forgery features and make full use of the label, we extend the famous self-supervised leaning framework MoCo~\cite{he2020momentum} to the fully-supervised version. 

Let $x_i\in{R^{H{\times}W\times3}}$ denote the input image.
We firstly generate two different views $v_1(x_i)$ and $v_2(x_i)$ with specially designed data augmentations. Then the $v_1(x_i)$ and $v_2(x_i)$ are fed into query encoder $f_q$ and momentum key encoder $f_k$
to obtain corresponding feature maps $f_q(v_1(x_i))$ and $f_q(v_2(x_i))\in R^{C \times H' \times W'}$. Then the framework is divided into two branches: supervised leaning branch and supervised contrastive learning branch.

\textbf{Supervised learning branch.  }

As shown in the top of the Fig~\ref{fig:main},
similar to the ordinary binary neural network, the class-wise logit $l \in {R^2}$ is obtained from query feature map by applying pooling operation and a single linear layer. Then we use the cross-entropy loss $L_{ce}$ between $l$ and $y_i$ to leverage the label information and make $f_q$ have basic discriminative ability.

\textbf{Contrastive learning branch.  }

This branch aims to arrange the distributions of feature space and further learn more general feature by feature contrasting.
Thus, query and key features need to be firstly generated as contrastive objects.
Different from the traditional contrastive framework which uses channel-wise feature as the query and key, due to the forgery clues usually hidden in the spatial dimensional,
we use $1\times1$ convolution operation to squeeze the channel dimensional while preserve the spatial dimensional and obtain the spatial-wise query $q \in R^{H'\times W'}$ and key $k\in R^{H'\times W'}$. Experiments result show that spatial feature is more useful than the channel feature.
After that,
\textit{supervised contrastive loss} and \textit{ self-similarity contrastive loss} is applied by the normalized query and key.

\textbf{Supervised contrastive loss.}
It aims to pull the normalized embedding of the positive pair closer than the negative pair on the hyperspherical plane. We use $\delta(u,v) = \frac{u}{||u||}.\frac{v}{||v||} $ denote the normalized cosine similarity. To construct the negative sample of corresponding query,
we also maintain two feature queues: hard real queue $M_{r}$ and hard fake queue $M_{f}$.
The details of the hard queues' generation are presented in Sec ~\ref{section:2}.
Our supervised contrastive loss which similar with the popular InfoNCE loss ~\cite{gutmann2010noise} can be written as: 
\begin{equation}
    L_{cl} = -\log\frac{e^{\delta(q,k) / \tau}}{e^{\delta(q,k)/ \tau} + \sum_{k_{m}\in K_{q}^{-}}e^{\delta(q,k_m)/ \tau}
    },
\end{equation}
where $\tau$ is a temperature parameter which controls the scale of distribution. $K_{q}^{-}$ represents the negative set of $q$, \textit{i.e.} $K_{q}^{-} = M_{f}$ when $q$ belongs to real while $K_{q}^{-} = M_{r}$ when $q$ belongs to fake.

Unlike existing common supervised contrastive leaning methods ~\cite{khosla2020supervised} which maximizes the invariance among the same category views, 
$L_{cl}$ only maximizes the invariance between two different views of single input to decoupling the impact of irrelevant forgery traces. Thus, the variance of the intra-class distributions can be guaranteed so that more transferability knowledge is preserved. 

\textbf{Self-similarity contrastive loss.}
Considering that fake faces are often partially changed, the feature similarities between the manipulated regions and the remaining regions are often very different ~\cite{chen2021local}. This phenomenon is widespread in various forgery face data set.
Thus, in addition to the comparison with other samples, we propose a self-similarity contrastive loss which enhance the inconsistency phenomenon of forgery face.

Specifically, $q$ is first transformed into 
$q^{'} \in R^{H^{'}W^{'}\times 1}$. Then the self-similarity feature is 
calculated based on the Gram matrices multiplication:
\begin{equation}
    s = q^{'} \odot q^{'T},
\end{equation}
here $s \in R^{H^{'}W^{'} \times H^{'}W^{'}}$. Then we labeled the $s$ into fake similarity $s_{f}$ and real similarity$s_{r}$ using ground truth within the single batch. Since $s$ represents the dense correlation
among spatial-wise feature $q$, we expect that the correlation of real features is greater than that of fake features.
Thus, the self-similarity contrastive loss can be designed as follows:
\begin{equation}
    % L_{sim} = -\log{\frac{\frac{1}{(H^{'}W^{'})^2} \sum {e^{s_{real} / \tau}}{}
    L_{smc} = -\log{\frac{e^{mean(s_{r})/ \tau}}{e^{mean(s_{r})/ \tau} + e^{mean(s_{f})/ \tau}}     },
\end{equation}
where $mean(.)$ represents the average operation.
$L_{smc}$ maximizes the similarity of the real feature while minimizes the fakes, which enhance the mining of inconsistent information and improve the generalization of the model.
% \begin{equation}
%     mean(s) = \frac{1}{(H^{'}W^{'})^2} \sum_{i=1}^{H^{'}W^{'}}\sum_{J=1}^{H^{'}W^{'}} s(i,j)
% \end{equation}
\subsection{Hard Sample Generation}
\label{section:2}
\citet{robinson2020contrastive,wang2021exploring} found that the hard negative pair selection is crucial for contrastive learning by experiments.
% and ~\citet{wang2021exploring} proved that
% harder negatives bring more gradient contributions than that the easy for the supervised contrastive learning. 
Meanwhile, \citet{sun2021domain} shows high-quality 
samples are more conducive to improving the generalization of the model. 
% Therefore, 
% Thus, how to select hard samples to build the memory queue is an important problem.

To simultaneously resolve the hard sample selection and high-quality sample selection, we propose a cross contrastive strategy.
Our key idea can be derived as: \textit{the more real the fake face is, the higher its quality and the higher its quality, the more it can be defined as a difficult sample.} Specifically, as shown in yellow dotted frame, we defined two prototypes for real and fake features, respectively. 
The prototypes are updated using EMA scheme defined as:
\begin{equation}
    P_{fake} = \alpha P_{fake} + (1-\alpha)k_{fake},
\end{equation}
\begin{equation}
    P_{real} = \alpha P_{real} + (1-\alpha)k_{real}.
\end{equation}
Then, we calculate the similarity of fake/fake feature and $P_{real}$/$P_{fake}$ as basis to decide whether the feature enqueue. More formally, the screening progress can be derived as:
\begin{equation}
    \label{equation:5}
    \left\{
    \begin{aligned}
        &\delta(k_{fake},P_{real}) > \theta  , &  k_{fake}->M_{f}\\
        &\delta(k_{real},P_{fake}) > \theta  , &  k_{real}->M_{r},
    \end{aligned}
    \right.
    \end{equation}
where $\theta$ is a threshold and the $->$ represents the enqueue operation.
\subsection{General Forgery Face Transform}
In the contrastive learning framework~\cite{he2020momentum}, a query matches a key if they are encoded views of the same image.
Since general face forgery detection task is very different with the common classification task such as face recognition, it is important to design a data transform strategy suitable for this task. We argue that the key of the general forgery face transform is to eliminate task-irrelevant contextual factors such as high-level face content, specific manipulated texture, background information \textit{e.t.c}. 
To address this issues, we design the following operations: 

\begin{itemize}
    \item \textbf{RandomPatch.} 
    Because face forgery detection mainly focuses on subtle manipulated traces rather than face content. Thus, we use random patch strategy to destroy the structure of the input face. Specifically, we divide the input face into $3 \times 3$ patches, and then randomly shuffle them. Both query and key streams can be used with a certain probability ($p_{rp} = 0.7$).
    \item \textbf{SRM.}
    ~\cite{luo2021generalizing} has proved that SRM noises~\cite{fridrich2012rich} can extract high-frequency features and boost the generalization ability.
    Take inspiration from this, we leverage the SRM operation as one of our data transform. Since SRM noises depress the most of the texture information and are very different from the RGB image, 
    we force this operation to appear in query stream and key stream at the same time with a certain probability ($p_{srm} = 0.3$).
    \item \textbf{Different Frame.}
    To reduce the influence of different expressions and motions on forged extraction, we choose different frames of the same video as contrast objective with a certain probability ($p_{df} = 0.5$).
    \item \textbf{Frequency Mixup}
    
    Since the manipulated clues are usually hidden in the high-frequency region, to extend the. 

    \item \textbf{Common Augmentation}
    In addition to the specially designed data transform, common data augmentation such as horizontal flip, random crop, Gaussian blur and Gaussian Noise.
\end{itemize}
\subsection{Overall Loss Function}
Considering both the cross entropy loss based supervised learning branch and two InfoNCE losses based contrastive learning branch, the overall loss for our proposed method is:
\begin{equation}
    L_{all} = \phi (L_{cl} +L_{smc}) + (1-\phi) L_{ce},
\end{equation}
where $\phi$ is the hyper-parameters used to balance the cross-entropy loss and contrastive loss.
\label{section:3}



==> trashword.tex <==

% $K_{q}^{-}$ and $K_{q}^{+}$represents the negative and positive sets of $q$, respectively. We use simple queue of the same category with query as $K+$ and use hard queue of the different category with query as $K-$.  
% $L_{cl}$ maximizes the invariance between two different views of single input which help to diverse the intra-class distributions and decoupling the impact of irrelevant forgery traces. 

% $L_{cl}^{'}$ maximizes the invariance between original and its same simple category views.
% closer while push the negative 
% to diverse the intra-class distributions and Learn from inconsistencies of forgery face, respectively.
% As mentioned in the introduction, to diverse the intra-class feature's distributions, we calculate the contrastive loss 

% \begin{equation}
%     L_{cl}^{'} = -\log\frac{\sum_{k_{n}\in K_{q}^{+}} e^{\delta(q,k_{n}) / \tau}}{\sum_{k_{n}\in K_{q}^{+}}e^{\delta(q,k_{n})/ \tau} + \sum_{k_{m}\in K_{q}^{-}}e^{\delta(q,k_m)/ \tau}
%     }
% \end{equation}

%and $y_i \in{\{0,1\}}$ represents the label of $x_i$.

%easy real queue $M_{r}^{e}$ easy fake queue $M_{f}^{e}$$L_{cl}$ maximizes the invariance between two different views of single input which help to diverse the intra-class distributions and decoupling the impact of irrelevant forgery traces. 



% Our proposed general forgery face transform aims to depress the influence of high-level face content, specific manipulated texture bias and background information \textit{e.t.c}. As shown in the left part of the Fig~\ref{fig:main}, our general forgery data augmentation contains four different operations:

$q$ is first flattened into one-dimensional vector and then inserted size one at the last position.



% a fake face is more like the real one, the quality is higher thus this sample is defined harder. Intuitively, the if a human can not

